EMF-Efficient MU-MIMO Networks: Harnessing Aerial RIS Technology

The rollout of the fifth-generation (5G) networks has raised some concerns about potential health effects from increased exposure to electromagnetic fields (EMF). To address these concerns, we design a novel EMF-aware architecture for uplink communications. Specifically, we propose an aerial reconfigurable intelligent surface (ARIS) assisted multi-user multiple-input multiple-output (MIMO) system, where the ARIS features a reconfigurable intelligent surface (RIS) panel mounted on an unmanned aerial vehicle (UAV), offering a flexible and adaptive solution for reducing uplink EMF exposure. We formulate and solve a new problem to minimize the EMF exposure by optimizing the system parameters, such as transmit beamforming, resource allocation, transmit power, ARIS phase shifts, and ARIS trajectory. Our numerical results demonstrate the effectiveness of EMF-aware transmission scheme over the benchmark methods, achieving EMF reductions of over 30% and 90% compared to the fixed ARIS and non-ARIS schemes, respectively.

==> Figures/ExpvsRISele/DinkelbachConv.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.53,0.4)}},legend cell align=left},
}
\begin{tikzpicture}
\begin{axis}[
    xlabel near ticks,
    ylabel near ticks,
    % grid=major,
    xlabel={Iteration},
    ylabel={$\lambda$ ($\times 10^{-13}$)},
    width=0.5\linewidth,
    legend style={fill=none},
    ylabel style={font=\normalsize},
    xlabel style={font=\normalsize},
    yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=3},
]

\addplot coordinates {
    (1, 1.669)
    (2, 1.382)
    (3, 1.382)
    (4, 1.382)
    (5, 1.382)
    (6, 1.382)
};
\end{axis}
\end{tikzpicture}

==> Figures/ExpvsRISele/EXPGa.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.53,0.4)}},legend cell align=left},
	% 	legend style={font=\footnotesize, at={(0.99,0.75)}}
} %
%\pgfplotsset{compat=1.18}
\begin{tikzpicture}
\begin{semilogyaxis}[
    xlabel near ticks,
    ylabel near ticks,
    grid=major,
    xlabel={$N$},
    ylabel={$\textrm{EI}$ (W/Kg)},
    width=0.5\linewidth,
    xmin=10,
    xmax=130,
    ytick={1e-2, 1e-3, 1e-4, 1e-5, 1e-6 },
    % ymin=1e-4,
    % ymax=0.1,
    legend style={fill=none},
    ylabel style={font=\normalsize},
    xlabel style={font=\normalsize},
    legend entries={random, proposed algorithm, genetic algorithm}
]
    \addplot[cyan] table {Figures/Exp vs RIS ele/ErndGa.dat};
    \addplot[red] table {Figures/Exp vs RIS ele/EhatGa.dat};
    \addplot[blue, dashed] table {Figures/Exp vs RIS ele/EGa.dat};
   
\end{semilogyaxis}
\end{tikzpicture}

==> Figures/Prx.tex <==
\pgfplotsset{every axis/.append style={
    font=\footnotesize,
    line width=1pt,
    legend style={fill opacity=0.5, % 
        draw opacity=1,  
        text opacity=1,      
font=\footnotesize,at={(0.78,0.82)}, anchor=south, legend columns=1}, % Move legend to upper left
    legend cell align=left
}}
\pgfplotsset{compat=1.18}

\definecolor{mycolor1}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor2}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor3}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor4}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{mycolor5}{rgb}{0.00000,0.44700,0.74100}%

\begin{tikzpicture}

\begin{semilogyaxis}[%
        yticklabel style={/pgf/number format/sci, /pgf/number format/fixed},
width = 0.5\columnwidth,
xmin =0.01,
xmax =0.99,
ymin = 10,
% ytick ={0.2,0.4,0.6,0.8,1},
grid = major,
%axis background/.style={fill=white},
% axis x line*=bottom,
% axis y line*=left,
% axis line style={->},
xlabel={$\gamma$},
ylabel={$f(\gamma)$},
]

 \addplot[very thick, blue,smooth] table {Figures/Prxratio.dat};
\addlegendentry{$\frac{1}{\gamma^2 (1-\gamma)^2}$}
\end{semilogyaxis}
\end{tikzpicture}%


==> TrajOpt.tex <==
Based on the optimal power allocation and the share of the achieved data rate between the assigned subcarrier for different time slots $\bar{r}_{u,n}[\ell]$, the individual exposure index at $l$ time is written as
\begin{equation}
    E_u(\pvl) = \sum_{n=1}^{N_c} \ \delta_{u,n}[\ell]\ \overline{\mathrm{SAR}}\left(\boldsymbol{\alpha}_{u, n} [\ell], \boldsymbol{\beta}_{u,n} [\ell]\right)\ (2^{\bar{r}_{u,n}[\ell]/w}-1)\frac{\sigma^2}{\gamma(\pvun [\ell])}.
\end{equation}
Again our problem is presented as minimizing the sum-of-ratio fractional programming. To solve this problem, we introduce auxiliary variables, $x_{u,n}[\ell], \forall u\in \mathcal{U}$, and we formulate the objective function using the quadratic transform technique as follow
\begin{subequations}
\label{41}
\begin{alignat}{3}
(\textrm{P5}) \quad &\underset{\boldsymbol{Q},\boldsymbol{X}}{\text{minimize}}        &\qquad& \phi(\mathbf{Q},\mathbf{X})\\
   &\text{subject to} &      & \boldsymbol{X}[\ell] \in \mathcal{R}^{U \times \nc}, \forall l \in \mathcal{N}_t, \label{Xconst}\\
   &                 &      & \eqref{UAV-dis} , \eqref{finalpoint},
   \end{alignat}
     \end{subequations}
where 
\begin{equation}
\phi(\mathbf{Q},\mathbf{X})\triangleq \sum^{N_T}_{l=1}\sum^{U}_{u=1} \sum^{N_c}_{n=1} \delta_{u,n}[\ell]\left( 2\ x_{u,n}[\ell] \ c_{u,n}[\ell] -x^2_{u,n}[\ell] \: \gamma(\pvun [\ell])\right).
\end{equation}
For a giving $Q$, the optimal $\hat{x}_{u,n}[\ell]$ at each iteration can be found in closed form as
\begin{equation}
\hat{x}_{u,n} [\ell] =\frac{c_{u,n}[\ell]}{\gamma(\hat{\pv}_{u,n} [\ell])} , \forall u \in \mathcal{U}, \forall n \in \mathcal{N}_c \text{ and } \forall l \in \mathcal{N}_T .
    \label{XTraj}
\end{equation}
The new equivalent problem is still non-convex with respect to the \ac{UAV} trajectory variables $\boldsymbol{Q}$. To show the dependency of the objective function on the \ac{ARIS} location, $\gamma(\pvun [\ell])$ is expressed differently as 
\begin{equation}
    \gamma(\pvun [\ell])=\frac{a_{u,n}[\ell]}{d_{u\text{R}}^{\kappa_1}[\ell]~d_{\text{RB}}^{\kappa_2}[\ell]} + \frac{b_{u,n}[\ell]}{\sqrt{d_{u\text{R}}^{\kappa_1}[\ell]~d_{\text{RB}}^{\kappa_2}[\ell]}},
\end{equation}
where $a_{u,n}[\ell]= \rho^2\ \| \bar{\boldsymbol{H}}^{\text{RB}}_n[\ell] \boldsymbol{\Theta}[\ell] \bar{\mathbf{h}}^{\text{uR}}_{u,n}[\ell]\|^2, b_{u,n}[\ell]= 2\ \rho \ \text{Re}(\boldsymbol{h}_{u,n}^d[\ell]^{\mathrm{H}} \bar{\boldsymbol{H}}^{\text{RB}}_n[\ell] \boldsymbol{\Theta}[\ell] \bar{\mathbf{h}}^{\text{uR}}_{u,n}[\ell]),$
\begin{align*}
    \bar{\boldsymbol{H}}^{\text{RB}}_n[\ell] &=\left(\sqrt{\frac{K_2}{K_2+1}} \bar{\boldsymbol{H}}^{\text{RB}}_n[\ell]+\sqrt{\frac{1}{K_2+1}} \tilde{\boldsymbol{H}}^{\text{RB}}_n[\ell]\right),
    \\
    \text{and }
    \bar{\mathbf{h}}^{\text{uR}}_{u,n}[\ell] &= \left(\sqrt{\frac{K_1}{K_1+1}} \bar{\mathbf{H}}^{\text{uR}}_{u,n}[\ell]+\sqrt{\frac{1}{K_1+1}} \tilde{\mathbf{H}}^{\text{uR}}_{u,n}[\ell]\right) \boldsymbol{f}_{u,n}[\ell].
\end{align*}
Note that the non-convexity of the subproblem comes from the coupling between the distances between users-\ac{ARIS} and \ac{ARIS}-\ac{BS}. Hence, we introduce new variables $\boldsymbol{u}_u$ and $\boldsymbol{v}$, and we consider new constraints to provide bounds on the distances between the users and the \ac{ARIS} and between the \ac{ARIS} and the \ac{BS} as follows
\begin{subequations}
    \begin{alignat}{2}
    & u_{u}[\ell] \geq d_{u\text{R}}[\ell],\forall u \in \mathcal{U} \label{d_uR} \text{ and } \forall l \in \mathcal{N_T},\\ 
    & v[\ell] \geq d_{\text{RB}}[\ell], \forall l \in \mathcal{N_T} \label{d_RB}.
    \end{alignat}
\end{subequations}
By introducing the auxiliary variables, we relax the non-convexity of the problem and we formulate it into a more tractable one. The equality at the optimal solution between the original and the new reformulated subproblem is guaranteed since increasing the value of the new slack variables reduces the objective value.
% \cite{}. later add ref 
After relaxation, $(\textrm{P5})$ can be reformulated as
\begin{subequations}
\label{45}
\begin{alignat}{2}
&\underset{\mathbf{Q,u,v}}{\text{minimize}}        &\qquad&  \sum_{l=0}^{N_T} \sum_{u=1}^{U} \sum_{n=1}^{N_c} 2 \ x_{u,n}[\ell]~ c_{u,n}[\ell]-x^2_{u,n}[\ell] \: \frac{a_{u,n}[\ell]}{u_u[\ell]^{\kappa_1}v[\ell]^{\kappa_2}}  + \frac{b_{u,n}[\ell]}{u_u[\ell]^{\frac{\kappa_1}{2}}v[\ell]^{\frac{\kappa_2}{2}}}\\
&\textrm{subject to}
&                 &    \eqref{Xconst},\eqref{d_uR}, \eqref{d_RB},\eqref{UAV-dis},\eqref{finalpoint}.
\end{alignat}
\end{subequations}
However, the problem is still non-convex. Therefore, \ac{SCA} method is used to optimize the trajectory.
Firstly, we derive the first-order Taylor approximation for the non-convex objective function and constraints at a given feasible points ($\mathbf{u}_{u}^{0}, \mathbf{v}^{0}$)
\begin{equation}
   x^2_{u,n}[\ell] \:\frac{a_{u,n}[\ell]}{u_u[\ell]^{\kappa_1}v[\ell]^{\kappa_2}}  + \frac{b_{u,n}[\ell]}{u_u[\ell]^{\frac{\kappa_1}{2}}v[\ell]^{\frac{\kappa_2}{2}}} \leq x^2_{u,n}[\ell] \left( A_{u,n}[\ell] + B_{u,n}[\ell] \right),
\end{equation}
\begin{subequations}
\begin{alignat}{2}
   & d_{u\text{R}}^2[\ell]+(u_{u}^{0}[\ell])^2   - 2~u_{u}^{0}[\ell]~ u_{u}[\ell]\leq 0, \forall u \in \mathcal{U} \text{ and } \forall l \in \mathcal{N}_T,  \\
   & d_{\text{RB}}^2[\ell]+(v^{0}[\ell])^2 - 2~v^{0}[\ell]~ v[\ell] \leq 0,\forall l \in \mathcal{N}_T,
   \end{alignat}
\end{subequations}
where 
\begin{equation}
  A_{u,n}[\ell] =a_{u,n}[\ell] \left(\frac{1}{(u_{u}^{0}[\ell])^{\kappa_1}+ (v^{0}[\ell])^{\kappa_2}}-\frac{\kappa_1 (u_u[\ell]-u_{u}^{0}[\ell])}{(u_{u}^{0}[\ell])^{\kappa_1 + 1}+ v[\ell]^{\kappa_2}} -\frac{\kappa_2 (v[\ell]-v^{0}[\ell])}{u_{u}[\ell]^{\kappa_1}+ (v^{0}[\ell])^{\kappa_2 +1} }\right) ,
\end{equation}
 and 
 \begin{equation}
     B_{u,n}[\ell] =b_{u,n}[\ell] \left(\frac{1}{(u_{u}^{0}[\ell])^{\frac{\kappa_1}{2} }+ (v^{0}[\ell])^{\frac{\kappa_2}{2}}}+\frac{\frac{-\kappa_1}{2} (u_u[\ell]-u_{u}^{0}[\ell])}{(u_{u}^{0}[\ell])^{\frac{\kappa_1}{2} + 1}+ v[\ell]^{\frac{\kappa_2}{2}}} -\frac{\frac{\kappa_2}{2} (v[\ell]-v^{0}[\ell])}{u_{u}[\ell]^{\frac{\kappa_1}{2}}+ (v^{0}[\ell])^{\frac{\kappa_2}{2} +1} }\right).
 \end{equation} 
 Based on the analysis above, the optimization problem of the \ac{ARIS} trajectory is approximated as follows
 \begin{subequations}
\begin{alignat}{3}
(\textrm{P5}^\prime) \quad  &\underset{\mathbf{Q,U,v}}{\text{minimize}}        & \qquad& \sum_{l=1}^{N_T} \sum_{u=1}^{U} \sum_{n=1}^{N_c} \delta_{u,n}[\ell] (2\,x_{u,n}[\ell]~ c_{u,n}[\ell]-x^2_{u,n}[\ell] \: (A_{u,n}[\ell] + B_{u,n}[\ell] ))\\
&\textrm{subject to}
& \qquad &\qquad    \eqref{Xconst},\eqref{d_uR}, \eqref{d_RB},\eqref{UAV-dis},\eqref{finalpoint}.
\end{alignat}
\end{subequations}
% Since the first-order Taylor approximation give us the global over-estimators, the initial problem and the reformulated one have the same optimal solution.
As a consequence, we note that the objective function and its feasible set are convex. Now, the problem is a convex optimization problem which can be solved efficiently using the convex solvers such as CVX.
% the global convergence is not guaranteed.
